EHRXQA: A Multi-Modal Question Answering Dataset for Electronic Health Records with Chest X-ray Images

Electronic Health Records (EHRs), which contain patients' medical histories in various multi-modal formats, often overlook the potential for joint reasoning across imaging and table modalities underexplored in current EHR Question Answering (QA) systems. In this paper, we introduce EHRXQA, a novel multi-modal question answering dataset combining structured EHRs and chest X-ray images. To develop our dataset, we first construct two uni-modal resources: 1) The MIMIC-CXR-VQA dataset, our newly created medical visual question answering (VQA) benchmark, specifically designed to augment the imaging modality in EHR QA, and 2) EHRSQL (MIMIC-IV), a refashioned version of a previously established table-based EHR QA dataset. By integrating these two uni-modal resources, we successfully construct a multi-modal EHR QA dataset that necessitates both uni-modal and cross-modal reasoning. To address the unique challenges of multi-modal questions within EHRs, we propose a NeuralSQL-based strategy equipped with an external VQA API. This pioneering endeavor enhances engagement with multi-modal EHR sources and we believe that our dataset can catalyze advances in real-world medical scenarios such as clinical decision-making and research. EHRXQA is available at https://github.com/baeseongsu/ehrxqa.

==> supp_tabs/ehrxqa_full_templates.tex <==
\begin{longtblr}
[
  caption = {Full list of 168 \textit{Image}-related question templates in EHRXQA},
  label = {tab:img_template_full},
]
{
  colspec = {X[c,m]X[c,m]X[c,m]X[10,l,m]},
  colsep = 0.3pt,
  rowhead = 1,
  hlines,
  rows={font=\scriptsize},
  rowsep=0.3pt,
}
\textbf{Patient scope} & \multicolumn{2}{c}{\textbf{Modality scope}} & \multicolumn{1}{c}{\textbf{Question Template}} \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any \$\{category\} in the \$\{object\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is there \$\{attribute\} in the \$\{object\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is the \$\{object\} abnormal? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any \$\{category\_1\} or \$\{category\_2\} in the \$\{object\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there both \$\{attribute\_1\} and \$\{attribute\_2\} in the \$\{object\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is there either \$\{attribute\_1\} or \$\{attribute\_2\} in the \$\{object\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all \$\{category\} in the \$\{object\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all abnormality in the \$\{object\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all \$\{category\_1\} and \$\{category\_2\} in the \$\{object\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], which \$\{category\} is related to the \$\{object\}, \$\{attribute\_1\} or \$\{attribute\_2\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any abnormality in either the \$\{object\_1\} or the \$\{object\_2\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any abnormality in both the \$\{object\_1\} and the \$\{object\_2\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all \$\{category\} in either the \$\{object\_1\} or the \$\{object\_2\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all common \$\{category\} in both the \$\{object\_1\} and the \$\{object\_2\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all \$\{category\} only in the \$\{object\_1\} but not in the \$\{object\_2\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all abnormality in either the \$\{object\_1\} or the \$\{object\_2\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all common abnormality in both the \$\{object\_1\} and the \$\{object\_2\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all abnormality only in the \$\{object\_1\} but not in the \$\{object\_2\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any \$\{category\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any abnormality? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any \$\{category\_1\} or \$\{category\_2\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is there \$\{attribute\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there both \$\{attribute\_1\} and \$\{attribute\_2\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is there either \$\{attribute\_1\} or \$\{attribute\_2\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all \$\{category\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all \$\{category\_1\} and \$\{category\_2\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all abnormality. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], which \$\{category\} is related, \$\{attribute\_1\} or \$\{attribute\_2\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are both the \$\{object\_1\} and the \$\{object\_2\} related to \$\{attribute\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is either the \$\{object\_1\} or the \$\{object\_2\} related to \$\{attribute\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all anatomical locations related to \$\{attribute\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], which anatomical location is related to \$\{attribute\}, the \$\{object\_1\} or the \$\{object\_2\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], which anatomical location is abnormal, the \$\{object\_1\} or the \$\{object\_2\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all anatomical locations related to either \$\{attribute\_1\} or \$\{attribute\_2\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all common anatomical locations related to both \$\{attribute\_1\} and \$\{attribute\_2\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all anatomical locations related to \$\{attribute\_1\} but not \$\{attribute\_2\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any \$\{category\} related to the \$\{object\_1\} and the \$\{object\_2\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any \$\{category\} related to the \$\{object\_1\} or the \$\{object\_2\}? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all anatomical locations related to any \$\{category\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all anatomical locations related to any \$\{category\_1\} or \$\{category\_2\}. \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is the width of the cardiac silhouette wider than 1/2 of the thorax width? \\
single & Image & 1-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is the width of the upper mediastinum wider than 1/3 of the thorax width? \\
single & Image & 1-image & Given the study \{study\_id\}, are there any \$\{category\} in the \$\{object\}? \\
single & Image & 1-image & Given the study \{study\_id\}, is there \$\{attribute\} in the \$\{object\}? \\
single & Image & 1-image & Given the study \{study\_id\}, is the \$\{object\} abnormal? \\
single & Image & 1-image & Given the study \{study\_id\}, are there any \$\{category\_1\} or \$\{category\_2\} in the \$\{object\}? \\
single & Image & 1-image & Given the study \{study\_id\}, are there both \$\{attribute\_1\} and \$\{attribute\_2\} in the \$\{object\}? \\
single & Image & 1-image & Given the study \{study\_id\}, is there either \$\{attribute\_1\} or \$\{attribute\_2\} in the \$\{object\}? \\
single & Image & 1-image & Given the study \{study\_id\}, list all \$\{category\} in the \$\{object\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all abnormality in the \$\{object\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all \$\{category\_1\} and \$\{category\_2\} in the \$\{object\}. \\
single & Image & 1-image & Given the study \{study\_id\}, which \$\{category\} is related to the \$\{object\}, \$\{attribute\_1\} or \$\{attribute\_2\}? \\
single & Image & 1-image & Given the study \{study\_id\}, are there any abnormality in either the \$\{object\_1\} or the \$\{object\_2\}? \\
single & Image & 1-image & Given the study \{study\_id\}, are there any abnormality in both the \$\{object\_1\} and the \$\{object\_2\}? \\
single & Image & 1-image & Given the study \{study\_id\}, list all \$\{category\} in either the \$\{object\_1\} or the \$\{object\_2\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all common \$\{category\} in both the \$\{object\_1\} and the \$\{object\_2\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all \$\{category\} only in the \$\{object\_1\} but not in the \$\{object\_2\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all abnormality in either the \$\{object\_1\} or the \$\{object\_2\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all common abnormality in both the \$\{object\_1\} and the \$\{object\_2\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all abnormality only in the \$\{object\_1\} but not in the \$\{object\_2\}. \\
single & Image & 1-image & Given the study \{study\_id\}, are there any \$\{category\}? \\
single & Image & 1-image & Given the study \{study\_id\}, are there any abnormality? \\
single & Image & 1-image & Given the study \{study\_id\}, are there any \$\{category\_1\} or \$\{category\_2\}? \\
single & Image & 1-image & Given the study \{study\_id\}, is there \$\{attribute\}? \\
single & Image & 1-image & Given the study \{study\_id\}, are there both \$\{attribute\_1\} and \$\{attribute\_2\}? \\
single & Image & 1-image & Given the study \{study\_id\}, is there either \$\{attribute\_1\} or \$\{attribute\_2\}? \\
single & Image & 1-image & Given the study \{study\_id\}, list all \$\{category\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all \$\{category\_1\} and \$\{category\_2\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all abnormality. \\
single & Image & 1-image & Given the study \{study\_id\}, which \$\{category\} is related, \$\{attribute\_1\} or \$\{attribute\_2\}? \\
single & Image & 1-image & Given the study \{study\_id\}, are both the \$\{object\_1\} and the \$\{object\_2\} related to \$\{attribute\}? \\
single & Image & 1-image & Given the study \{study\_id\}, is either the \$\{object\_1\} or the \$\{object\_2\} related to \$\{attribute\}? \\
single & Image & 1-image & Given the study \{study\_id\}, list all anatomical locations related to \$\{attribute\}. \\
single & Image & 1-image & Given the study \{study\_id\}, which anatomical location is related to \$\{attribute\}, the \$\{object\_1\} or the \$\{object\_2\}? \\
single & Image & 1-image & Given the study \{study\_id\}, which anatomical location is abnormal, the \$\{object\_1\} or the \$\{object\_2\}? \\
single & Image & 1-image & Given the study \{study\_id\}, list all anatomical locations related to either \$\{attribute\_1\} or \$\{attribute\_2\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all common anatomical locations related to both \$\{attribute\_1\} and \$\{attribute\_2\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all anatomical locations related to \$\{attribute\_1\} but not \$\{attribute\_2\}. \\
single & Image & 1-image & Given the study \{study\_id\}, are there any \$\{category\} related to the \$\{object\_1\} and the \$\{object\_2\}? \\
single & Image & 1-image & Given the study \{study\_id\}, are there any \$\{category\} related to the \$\{object\_1\} or the \$\{object\_2\}? \\
single & Image & 1-image & Given the study \{study\_id\}, list all anatomical locations related to any \$\{category\}. \\
single & Image & 1-image & Given the study \{study\_id\}, list all anatomical locations related to any \$\{category\_1\} or \$\{category\_2\}. \\
single & Image & 1-image & Given the study \{study\_id\}, is the width of the cardiac silhouette wider than 1/2 of the thorax width? \\
single & Image & 1-image & Given the study \{study\_id\}, is the width of the upper mediastinum wider than 1/3 of the thorax width? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any \$\{category\} that are \$\{comparison\} in the \$\{object\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is \$\{attribute\} \$\{comparison\} in the \$\{object\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any abnormality that are \$\{comparison\} in the \$\{object\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any \$\{category\} that are \$\{comparison\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any abnormality that are \$\{comparison\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is \$\{attribute\} \$\{comparison\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all \$\{category\} that are \$\{comparison\} in the \$\{object\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all abnormality that are \$\{comparison\} in the \$\{object\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all \$\{category\} that are \$\{comparison\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all abnormality that are \$\{comparison\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all anatomical locations related to \$\{attribute\} that are \$\{comparison\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all anatomical locations related to any \$\{category\} that are \$\{comparison\} compared to the [time\_filter\_exact2] study of patient \{patient\_id\} [time\_filter\_global2]? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any \$\{category\} that are \$\{comparison\} in the \$\{object\} compared to the previous study? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is \$\{attribute\} \$\{comparison\} in the \$\{object\} compared to the previous study? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any abnormality that are \$\{comparison\} in the \$\{object\} compared to the previous study? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any \$\{category\} that are \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], are there any abnormality that are \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], is \$\{attribute\} \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all \$\{category\} that are \$\{comparison\} in the \$\{object\} compared to the previous study? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all abnormality that are \$\{comparison\} in the \$\{object\} compared to the previous study? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all \$\{category\} that are \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all abnormality that are \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all anatomical locations related to \$\{attribute\} that are \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the [time\_filter\_exact1] study of patient \{patient\_id\} [time\_filter\_global1], list all anatomical locations related to any \$\{category\} that are \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, are there any \$\{category\} that are \$\{comparison\} in the \$\{object\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, is \$\{attribute\} \$\{comparison\} in the \$\{object\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, are there any abnormality that are \$\{comparison\} in the \$\{object\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, are there any \$\{category\} that are \$\{comparison\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, are there any abnormality that are \$\{comparison\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, is \$\{attribute\} \$\{comparison\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all \$\{category\} that are \$\{comparison\} in the \$\{object\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all abnormality that are \$\{comparison\} in the \$\{object\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all \$\{category\} that are \$\{comparison\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all abnormality that are \$\{comparison\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all anatomical locations related to \$\{attribute\} that are \$\{comparison\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all anatomical locations related to any \$\{category\} that are \$\{comparison\} compared to the \{study\_id2\} study? \\
single & Image & 2-image & Given the \{study\_id1\} study, are there any \$\{category\} that are \$\{comparison\} in the \$\{object\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, is \$\{attribute\} \$\{comparison\} in the \$\{object\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, are there any abnormality that are \$\{comparison\} in the \$\{object\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, are there any \$\{category\} that are \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, are there any abnormality that are \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, is \$\{attribute\} \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all \$\{category\} that are \$\{comparison\} in the \$\{object\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all abnormality that are \$\{comparison\} in the \$\{object\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all \$\{category\} that are \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all abnormality that are \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all anatomical locations related to \$\{attribute\} that are \$\{comparison\} compared to the previous study? \\
single & Image & 2-image & Given the \{study\_id1\} study, list all anatomical locations related to any \$\{category\} that are \$\{comparison\} compared to the previous study? \\
single & Image & N-image & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1]? \\
single & Image & N-image & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} had a chest X-ray study indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1]? \\
single & Image & N-image & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} had a chest X-ray study indicating any abnormality in the \$\{object\} [time\_filter\_global1]? \\
single & Image & N-image & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} had a chest X-ray study indicating \$\{attribute\} [time\_filter\_global1]? \\
single & Image & N-image & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} had a chest X-ray study indicating any \$\{category\} [time\_filter\_global1]? \\
single & Image & N-image & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} had a chest X-ray study indicating any abnormality [time\_filter\_global1]? \\
single & Image & N-image & When was the [time\_filter\_exact1] time that patient \{patient\_id\} had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1]? \\
single & Image & N-image & When was the [time\_filter\_exact1] time that patient \{patient\_id\} had a chest X-ray study indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1]? \\
single & Image & N-image & When was the [time\_filter\_exact1] time that patient \{patient\_id\} had a chest X-ray study indicating any abnormality in the \$\{object\} [time\_filter\_global1]? \\
single & Image & N-image & When was the [time\_filter\_exact1] time that patient \{patient\_id\} had a chest X-ray study indicating \$\{attribute\} [time\_filter\_global1]? \\
single & Image & N-image & When was the [time\_filter\_exact1] time that patient \{patient\_id\} had a chest X-ray study indicating any \$\{category\} [time\_filter\_global1]? \\
single & Image & N-image & When was the [time\_filter\_exact1] time that patient \{patient\_id\} had a chest X-ray study indicating any abnormality [time\_filter\_global1]? \\
single & Image & N-image & Has \{patient\_id\} had any chest X-ray study indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1]? \\
single & Image & N-image & Has \{patient\_id\} had any chest X-ray study indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1]? \\
single & Image & N-image & Has \{patient\_id\} had any chest X-ray study indicating any abnormality in the \$\{object\} [time\_filter\_global1]? \\
single & Image & N-image & Has \{patient\_id\} had any chest X-ray study indicating \$\{attribute\} [time\_filter\_global1]? \\
single & Image & N-image & Has \{patient\_id\} had any chest X-ray study indicating any \$\{category\} [time\_filter\_global1]? \\
single & Image & N-image & Has \{patient\_id\} had any chest X-ray study indicating any abnormality [time\_filter\_global1]? \\
single & Image & N-image & Count the number of times that patient \{patient\_id\} had chest X-ray studies indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1]. \\
single & Image & N-image & Count the number of times that patient \{patient\_id\} had chest X-ray studies indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1]. \\
single & Image & N-image & Count the number of times that patient \{patient\_id\} had chest X-ray studies indicating any abnormality in the \$\{object\} [time\_filter\_global1]. \\
single & Image & N-image & Count the number of times that patient \{patient\_id\} had chest X-ray studies indicating \$\{attribute\} [time\_filter\_global1]. \\
single & Image & N-image & Count the number of times that patient \{patient\_id\} had chest X-ray studies indicating any \$\{category\} [time\_filter\_global1]. \\
single & Image & N-image & Count the number of times that patient \{patient\_id\} had chest X-ray studies indicating any abnormality [time\_filter\_global1]. \\
group & Image & N-image & Count the number of patients who had any chest X-ray study indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image & N-image & Count the number of patients who had any chest X-ray study indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image & N-image & Count the number of patients who had any chest X-ray study indicating any abnormality in the \$\{object\} [time\_filter\_global1]. \\
group & Image & N-image & Count the number of patients who had any chest X-ray study indicating \$\{attribute\} [time\_filter\_global1]. \\
group & Image & N-image & Count the number of patients who had any chest X-ray study indicating any \$\{category\} [time\_filter\_global1]. \\
group & Image & N-image & Count the number of patients who had any chest X-ray study indicating any abnormality [time\_filter\_global1]. \\
group & Image & N-image & List the IDs of patients who had any chest X-ray study indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image & N-image & List the IDs of patients who had any chest X-ray study indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image & N-image & List the IDs of patients who had any chest X-ray study indicating any abnormality in the \$\{object\} [time\_filter\_global1]. \\
group & Image & N-image & List the IDs of patients who had any chest X-ray study indicating \$\{attribute\} [time\_filter\_global1]. \\
group & Image & N-image & List the IDs of patients who had any chest X-ray study indicating any \$\{category\} [time\_filter\_global1]. \\
group & Image & N-image & List the IDs of patients who had any chest X-ray study indicating any abnormality [time\_filter\_global1]. \\
\end{longtblr}

\begin{longtblr}
[
  caption = {Full list of 183 \textit{Table}-related question templates in EHRXQA},
  label = {tab:tab_template_full},
]
{
  colspec = {X[c,m]X[1.2,c,m]X[10,l,m]},
  colsep = 0.3pt,
  rowhead = 1,
  hlines,
  rows={font=\scriptsize},
  rowsep=0.3pt,
}
\textbf{Patient scope} & \begin{tabular}[c]{@{}c@{}}\textbf{Modality}\\\textbf{scope}\end{tabular} & \multicolumn{1}{c}{\textbf{Question Template}} \\
none & Table & What is the intake method of \{drug\_name\}? \\
none & Table & What is the cost of a procedure named \{procedure\_name\}? \\
none & Table & What is the cost of a \{lab\_name\} lab test? \\
none & Table & What is the cost of a drug named \{drug\_name\}? \\
none & Table & What is the cost of diagnosing \{diagnosis\_name\}? \\
none & Table & What does \{abbreviation\} stand for? \\
single & Table & What is the gender of patient \{patient\_id\}? \\
single & Table & What is the date of birth of patient \{patient\_id\}? \\
single & Table & What was the [time\_filter\_exact1] length of hospital stay of patient \{patient\_id\}? \\
single & Table & What is the change in the weight of patient \{patient\_id\} from the [time\_filter\_exact2] value measured [time\_filter\_global2] compared to the [time\_filter\_exact1] value measured [time\_filter\_global1]? \\
single & Table & What is the change in the value of \{lab\_name\} of patient \{patient\_id\} from the [time\_filter\_exact2] value measured [time\_filter\_global2] compared to the [time\_filter\_exact1] value measured [time\_filter\_global1]? \\
single & Table & What is the change in the \{vital\_name\} of patient \{patient\_id\} from the [time\_filter\_exact2] value measured [time\_filter\_global2] compared to the [time\_filter\_exact1] value measured [time\_filter\_global1]? \\
single & Table & Is the value of \{lab\_name\} of patient \{patient\_id\} [time\_filter\_exact2] measured [time\_filter\_global2] [comparison] than the [time\_filter\_exact1] value measured [time\_filter\_global1]? \\
single & Table & Is the \{vital\_name\} of patient \{patient\_id\} [time\_filter\_exact2] measured [time\_filter\_global2] [comparison] than the [time\_filter\_exact1] value measured [time\_filter\_global1]? \\
single & Table & What is\_verb the age of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What is\_verb the name of insurance of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What is\_verb the marital status of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What percentile is the value of \{lab\_value\} in a \{lab\_name\} lab test among patients of the same age as patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & How many [unit\_count] have passed since patient \{patient\_id\} was admitted to the hospital currently? \\
single & Table & How many [unit\_count] have passed since patient \{patient\_id\} was admitted to the ICU currently? \\
single & Table & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} was transferred to careunit \{careunit\} on the current hospital visit? \\
single & Table & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} was transferred to ward \{ward\_id\} on the current hospital visit? \\
single & Table & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} received a procedure on the current hospital visit? \\
single & Table & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} received a \{procedure\_name\} procedure on the current hospital visit? \\
single & Table & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} was diagnosed with \{diagnosis\_name\} on the current hospital visit? \\
single & Table & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} was prescribed \{drug\_name\} on the current hospital visit? \\
single & Table & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} received a \{lab\_name\} lab test on the current hospital visit? \\
single & Table & How many [unit\_count] have passed since the [time\_filter\_exact1] time patient \{patient\_id\} had a \{intake\_name\} intake on the current ICU visit? \\
single & Table & What was the [time\_filter\_exact1] hospital admission type of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the [time\_filter\_exact1] ward of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the [time\_filter\_exact1] careunit of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the [time\_filter\_exact1] measured height of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the [time\_filter\_exact1] measured weight of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the name of the diagnosis that patient \{patient\_id\} [time\_filter\_exact1] received [time\_filter\_global1]? \\
single & Table & What was the name of the procedure that patient \{patient\_id\} [time\_filter\_exact1] received [time\_filter\_global1]? \\
single & Table & What was the name of the drug that patient \{patient\_id\} was [time\_filter\_exact1] prescribed via \{drug\_route\} route [time\_filter\_global1]? \\
single & Table & What was the name of the drug that patient \{patient\_id\} was [time\_filter\_exact1] prescribed [time\_filter\_global1]? \\
single & Table & What was the name of the drug that patient \{patient\_id\} was prescribed [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
single & Table & What was the name of the drug that patient \{patient\_id\} was prescribed [time\_filter\_within] after having received a \{procedure\_name\} procedure [time\_filter\_global1]? \\
single & Table & What was the dose of \{drug\_name\} that patient \{patient\_id\} was [time\_filter\_exact1] prescribed [time\_filter\_global1]? \\
single & Table & What was the total amount of dose of \{drug\_name\} that patient \{patient\_id\} were prescribed [time\_filter\_global1]? \\
single & Table & What was the name of the drug that patient \{patient\_id\} were prescribed [n\_times] [time\_filter\_global1]? \\
single & Table & What is the new prescription of patient \{patient\_id\} [time\_filter\_global2] compared to the prescription [time\_filter\_global1]? \\
single & Table & What was the [time\_filter\_exact1] measured value of a \{lab\_name\} lab test of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the name of the lab test that patient \{patient\_id\} [time\_filter\_exact1] received [time\_filter\_global1]? \\
single & Table & What was the [agg\_function] \{lab\_name\} value of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the name of the allergy that patient \{patient\_id\} had [time\_filter\_global1]? \\
single & Table & What was the name of the substance that patient \{patient\_id\} was allergic to [time\_filter\_global1]? \\
single & Table & What was the organism name found in the [time\_filter\_exact1] \{culture\_name\} microbiology test of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the organism name found in the [time\_filter\_exact1] \{test\_name\} test of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the name of the specimen that patient \{patient\_id\} was [time\_filter\_exact1] tested [time\_filter\_global1]? \\
single & Table & What was the name of the microbiology test that patient \{patient\_id\} [time\_filter\_exact1] received [time\_filter\_global1]? \\
single & Table & What was the name of the intake that patient \{patient\_id\} [time\_filter\_exact1] had [time\_filter\_global1]? \\
single & Table & What was the total volume of \{intake\_name\} intake that patient \{patient\_id\} received [time\_filter\_global1]? \\
single & Table & What was the total volume of intake that patient \{patient\_id\} received [time\_filter\_global1]? \\
single & Table & What was the name of the output that patient \{patient\_id\} [time\_filter\_exact1] had [time\_filter\_global1]? \\
single & Table & What was the total volume of \{output\_name\} output that patient \{patient\_id\} had [time\_filter\_global1]? \\
single & Table & What was the total volume of output that patient \{patient\_id\} had [time\_filter\_global1]? \\
single & Table & What is the difference between the total volume of intake and output of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the [time\_filter\_exact1] measured \{vital\_name\} of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the [agg\_function] \{vital\_name\} of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What is\_verb the total hospital cost of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] hospital admission time of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] hospital admission time that patient \{patient\_id\} was admitted via \{admission\_route\} [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] hospital discharge time of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & What was the [time\_filter\_exact1] length of ICU stay of patient \{patient\_id\}? \\
single & Table & When was the [time\_filter\_exact1] time that patient \{patient\_id\} was diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] procedure time of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] time that patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] prescription time of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] time that patient \{patient\_id\} was prescribed \{drug\_name\} [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] time that patient \{patient\_id\} was prescribed \{drug\_name1\} and \{drug\_name2\} [time\_filter\_within] [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] time that patient \{patient\_id\} was prescribed a medication via \{drug\_route\} route [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] lab test of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] time that patient \{patient\_id\} received a \{lab\_name\} lab test [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] time that patient \{patient\_id\} had the [sort] value of \{lab\_name\} [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] microbiology test of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & When was patient \{patient\_id\}'s [time\_filter\_exact1] \{culture\_name\} microbiology test [time\_filter\_global1]? \\
single & Table & When was patient \{patient\_id\}'s [time\_filter\_exact1] \{test\_name\} test [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] time that patient \{patient\_id\} had a \{intake\_name\} intake [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] intake time of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] time that patient \{patient\_id\} had a \{output\_name\} output [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] time that patient \{patient\_id\} had a \{vital\_name\} measured [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] time that the \{vital\_name\} of patient \{patient\_id\} was [comparison] than \{vital\_value\} [time\_filter\_global1]? \\
single & Table & When was the [time\_filter\_exact1] time that patient \{patient\_id\} had the [sort] \{vital\_name\} [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure in other than the current hospital [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} been admitted to the hospital [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} been to an emergency room [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} received any procedure [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_global1]? \\
single & Table & What was the name of the procedure that patient \{patient\_id\} received [n\_times] [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} received any diagnosis [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} been prescribed \{drug\_name1\}, \{drug\_name2\}, or \{drug\_name3\} [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} been prescribed any medication [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} been prescribed \{drug\_name\} [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} received any lab test [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} received a \{lab\_name\} lab test [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} had any allergy [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} had any microbiology test result [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} had any \{culture\_name\} microbiology test result [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} had any \{test\_name\} test result [time\_filter\_global1]? \\
single & Table & Has\_verb there been any organism found in the [time\_filter\_exact1] \{culture\_name\} microbiology test of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & Has\_verb there been any organism found in the [time\_filter\_exact1] \{test\_name\} test of patient \{patient\_id\} [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} had any \{intake\_name\} intake [time\_filter\_global1]? \\
single & Table & Has\_verb patient \{patient\_id\} had any \{output\_name\} output [time\_filter\_global1]? \\
single & Table & Has\_verb the \{vital\_name\} of patient \{patient\_id\} been ever [comparison] than \{vital\_value\} [time\_filter\_global1]? \\
single & Table & Has\_verb the \{vital\_name\} of patient \{patient\_id\} been normal [time\_filter\_global1]? \\
single & Table & List the hospital admission time of patient \{patient\_id\} [time\_filter\_global1]. \\
single & Table & List the [unit\_average] [agg\_function] \{lab\_name\} lab value of patient \{patient\_id\} [time\_filter\_global1]. \\
single & Table & List the [unit\_average] [agg\_function] weight of patient \{patient\_id\} [time\_filter\_global1]. \\
single & Table & List the [unit\_average] [agg\_function] volume of \{intake\_name\} intake that patient \{patient\_id\} received [time\_filter\_global1]. \\
single & Table & List the [unit\_average] [agg\_function] volume of \{output\_name\} output that patient \{patient\_id\} had [time\_filter\_global1]. \\
single & Table & List the [unit\_average] [agg\_function] \{vital\_name\} of patient \{patient\_id\} [time\_filter\_global1]. \\
single & Table & Count the number of hospital visits of patient \{patient\_id\} [time\_filter\_global1]. \\
single & Table & Count the number of ICU visits of patient \{patient\_id\} [time\_filter\_global1]. \\
single & Table & Count the number of times that patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_global1]. \\
single & Table & Count the number of drugs patient \{patient\_id\} were prescribed [time\_filter\_global1]. \\
single & Table & Count the number of times that patient \{patient\_id\} were prescribed \{drug\_name\} [time\_filter\_global1]. \\
single & Table & Count the number of times that patient \{patient\_id\} received a \{lab\_name\} lab test [time\_filter\_global1]. \\
single & Table & Count the number of times that patient \{patient\_id\} had a \{intake\_name\} intake [time\_filter\_global1]. \\
single & Table & Count the number of times that patient \{patient\_id\} had a \{output\_name\} output [time\_filter\_global1]. \\
group & Table & Count the number of current patients. \\
group & Table & Count the number of current patients aged [age\_group]. \\
group & Table & What is the [n\_survival\_period] survival rate of patients diagnosed with \{diagnosis\_name\}? \\
group & Table & What is the [n\_survival\_period] survival rate of patients who were prescribed \{drug\_name\} after having been diagnosed with \{diagnosis\_name\}? \\
group & Table & What are the top [n\_rank] diagnoses that have the highest [n\_survival\_period] mortality rate? \\
group & Table & What is\_verb the [agg\_function] total hospital cost that involves a procedure named \{procedure\_name\} [time\_filter\_global1]? \\
group & Table & What is\_verb the [agg\_function] total hospital cost that involves a \{lab\_name\} lab test [time\_filter\_global1]? \\
group & Table & What is\_verb the [agg\_function] total hospital cost that involves a drug named \{drug\_name\} [time\_filter\_global1]? \\
group & Table & What is\_verb the [agg\_function] total hospital cost that involves a diagnosis named \{diagnosis\_name\} [time\_filter\_global1]? \\
group & Table & List the IDs of patients diagnosed with \{diagnosis\_name\} [time\_filter\_global1]. \\
group & Table & What is the [agg\_function] [unit\_average] number of patient records diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
group & Table & Count the number of patients who were dead after having been diagnosed with \{diagnosis\_name\} [time\_filter\_within] [time\_filter\_global1]. \\
group & Table & Count the number of patients who did not come back to the hospital [time\_filter\_within] after diagnosed with \{diagnosis\_name\} [time\_filter\_global1]. \\
group & Table & Count the number of patients who were admitted to the hospital [time\_filter\_global1]. \\
group & Table & Count the number of patients who were discharged from the hospital [time\_filter\_global1]. \\
group & Table & Count the number of patients who stayed in ward \{ward\_id\} [time\_filter\_global1]. \\
group & Table & Count the number of patients who stayed in careunit \{careunit\} [time\_filter\_global1]. \\
group & Table & Count the number of patients who were diagnosed with \{diagnosis\_name\} [time\_filter\_within] after having received a \{procedure\_name\} procedure [time\_filter\_global1]. \\
group & Table & Count the number of patients who were diagnosed with \{diagnosis\_name2\} [time\_filter\_within] after having been diagnosed with \{diagnosis\_name1\} [time\_filter\_global1]. \\
group & Table & Count the number of patients who were diagnosed with \{diagnosis\_name\} [time\_filter\_global1]. \\
group & Table & Count the number of patients who received a \{procedure\_name\} procedure [time\_filter\_global1]. \\
group & Table & Count the number of patients who received a \{procedure\_name\} procedure [n\_times] [time\_filter\_global1]. \\
group & Table & Count the number of patients who received a \{procedure\_name2\} procedure [time\_filter\_within] after having received a \{procedure\_name1\} procedure [time\_filter\_global1]. \\
group & Table & Count the number of patients who received a \{procedure\_name\} procedure [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]. \\
group & Table & Count the number of \{procedure\_name\} procedure cases [time\_filter\_global1]. \\
group & Table & Count the number of patients who were prescribed \{drug\_name\} [time\_filter\_global1]. \\
group & Table & Count the number of \{drug\_name\} prescription cases [time\_filter\_global1]. \\
group & Table & Count the number of patients who were prescribed \{drug\_name\} [time\_filter\_within] after having received a \{procedure\_name\} procedure [time\_filter\_global1]. \\
group & Table & Count the number of patients who were prescribed \{drug\_name\} [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]. \\
group & Table & Count the number of patients who received a \{lab\_name\} lab test [time\_filter\_global1]. \\
group & Table & Count the number of patients who received a \{culture\_name\} microbiology test [time\_filter\_global1]. \\
group & Table & Count the number of patients who received a \{test\_name\} test [time\_filter\_global1]. \\
group & Table & Count the number of patients who had a \{intake\_name\} intake [time\_filter\_global1]. \\
group & Table & What are\_verb the top [n\_rank] frequent diagnoses [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent diagnoses of patients aged [age\_group] [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent diagnoses that patients were diagnosed [time\_filter\_within] after having received a \{procedure\_name\} procedure [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent diagnoses that patients were diagnosed [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent procedures [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent procedures of patients aged [age\_group] [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent procedures that patients received [time\_filter\_within] after having received a \{procedure\_name\} procedure [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent procedures that patients received [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequently prescribed drugs [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequently prescribed drugs of patients aged [age\_group] [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent prescribed drugs for patients who were also prescribed \{drug\_name\} at the same time [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent drugs that patients were prescribed [time\_filter\_within] after having been prescribed with \{drug\_name\} [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequently prescribed drugs that patients were prescribed [time\_filter\_within] after having received a \{procedure\_name\} procedure [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequently prescribed drugs that patients were prescribed [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequently prescribed drugs that patients aged [age\_group] were prescribed [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequently prescribed drugs that \{gender\} patients aged [age\_group] were prescribed [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent lab tests [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent lab tests of patients aged [age\_group] [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent lab tests that patients had [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent lab tests that patients had [time\_filter\_within] after having received a \{procedure\_name\} procedure [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent specimens tested [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent microbiology tests [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent specimens that patients were tested [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent microbiology tests that patients had [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent specimens that patients were tested [time\_filter\_within] after having received a \{procedure\_name\} procedure [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent microbiology tests that patients had [time\_filter\_within] after having received a \{procedure\_name\} procedure [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent intake events [time\_filter\_global1]? \\
group & Table & What are\_verb the top [n\_rank] frequent output events [time\_filter\_global1]? \\
\end{longtblr}





\begin{longtblr}
[
  caption = {Full list of 96 \textit{Image+Table}-related question templates in EHRXQA},
  label = {tab:mm_template_full},
]
{
  colspec = {X[c,m]X[1.4,c,m]X[10,l,m]},
  colsep = 0.3pt,
  rowhead = 1,
  hlines,
  rows={font=\scriptsize},
  rowsep=0.3pt,
}
\textbf{Patient scope} & \begin{tabular}[c]{@{}c@{}}\textbf{Modality}\\\textbf{scope}\end{tabular} & \multicolumn{1}{c}{\textbf{Question Template}} \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any diagnosis [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any diagnosis [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any diagnosis [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any diagnosis [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any diagnosis [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any diagnosis [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any procedure [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any procedure [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any procedure [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any procedure [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any procedure [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received any procedure [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed any medication [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed any medication [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed any medication [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality in the \$\{object\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed any medication [time\_filter\_global1] and also had a chest X-ray study indicating \$\{attribute\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed any medication [time\_filter\_global1] and also had a chest X-ray study indicating any \$\{category\} within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed any medication [time\_filter\_global1] and also had a chest X-ray study indicating any abnormality within the same period? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any \$\{category\} in the \$\{object\} [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any abnormality in the \$\{object\} [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating \$\{attribute\} [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any \$\{category\} [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any abnormality [time\_filter\_within] after having been diagnosed with \{diagnosis\_name\} [time\_filter\_global1]? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} [time\_filter\_within] after having received \{procedure\_name\} procedure [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any \$\{category\} in the \$\{object\} [time\_filter\_within] after having received \{procedure\_name\} procedure [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any abnormality in the \$\{object\} [time\_filter\_within] after having received \{procedure\_name\} procedure [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating \$\{attribute\} [time\_filter\_within] after having received \{procedure\_name\} procedure [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any \$\{category\} [time\_filter\_within] after having received \{procedure\_name\} procedure [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any abnormality [time\_filter\_within] after having received \{procedure\_name\} procedure [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} [time\_filter\_within] after having been prescribed with \{drug\_name\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any \$\{category\} in the \$\{object\} [time\_filter\_within] after having been prescribed with \{drug\_name\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any abnormality in the \$\{object\} [time\_filter\_within] after having been prescribed with \{drug\_name\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating \$\{attribute\} [time\_filter\_within] after having been prescribed with \{drug\_name\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any \$\{category\} [time\_filter\_within] after having been prescribed with \{drug\_name\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} had a chest X-ray study indicating any abnormality [time\_filter\_within] after having been prescribed with \{drug\_name\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_within] after having had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_within] after having had a chest X-ray study indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_within] after having had a chest X-ray study indicating any abnormality in the \$\{object\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_within] after having had a chest X-ray study indicating \$\{attribute\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_within] after having had a chest X-ray study indicating any \$\{category\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been diagnosed with \{diagnosis\_name\} [time\_filter\_within] after having had a chest X-ray study indicating any abnormality [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_within] after having had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_within] after having had a chest X-ray study indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_within] after having had a chest X-ray study indicating any abnormality in the \$\{object\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_within] after having had a chest X-ray study indicating \$\{attribute\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_within] after having had a chest X-ray study indicating any \$\{category\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} received a \{procedure\_name\} procedure [time\_filter\_within] after having had a chest X-ray study indicating any abnormality [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_within] after having had a chest X-ray study indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_within] after having had a chest X-ray study indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_within] after having had a chest X-ray study indicating any abnormality in the \$\{object\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_within] after having had a chest X-ray study indicating \$\{attribute\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_within] after having had a chest X-ray study indicating any \$\{category\} [time\_filter\_global1] ? \\
single & Image + Table &  Has\_verb patient \{patient\_id\} been prescribed with \{drug\_name\} [time\_filter\_within] after having had a chest X-ray study indicating any abnormality [time\_filter\_global1] ? \\
group & Image + Table &  Count the number of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  Count the number of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  Count the number of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any abnormality in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  Count the number of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating \$\{attribute\} [time\_filter\_global1]. \\
group & Image + Table &  Count the number of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any \$\{category\} [time\_filter\_global1]. \\
group & Image + Table &  Count the number of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any abnormality [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any abnormality in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating \$\{attribute\} [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any \$\{category\} [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any abnormality [time\_filter\_global1]. \\
group & Image + Table &  Count the number of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  Count the number of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  Count the number of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any abnormality in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  Count the number of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating \$\{attribute\} [time\_filter\_global1]. \\
group & Image + Table &  Count the number of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any \$\{category\} [time\_filter\_global1]. \\
group & Image + Table &  Count the number of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any abnormality [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating \$\{attribute\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any \$\{category\} in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any abnormality in the \$\{object\} [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating \$\{attribute\} [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any \$\{category\} [time\_filter\_global1]. \\
group & Image + Table &  List the IDs of \{gender\} patients aged [age\_group] who had a chest X-ray study during hospital visit indicating any abnormality [time\_filter\_global1]. 
\end{longtblr}





==> supp_tabs/vqa_exp_template.tex <==
\begin{table}[H]
    \setlength{\tabcolsep}{3pt}
    \noindent
    \centering
        \captionsetup{font={small}}
        \caption{Comparison of performance of models on \textbf{MIMIC-CXR-VQA (\textit{Template})}. 
        }
        \resizebox{0.4\linewidth}{!}{%
            \begin{tabular}{@{}cccccc@{}}
            \toprule
            \multirow{2}{*}{Model} & \multicolumn{2}{c}{Valid} & \multicolumn{2}{c}{Test} \\ \cmidrule(l){2-5}
                                   & Acc & F1 (micro) & Acc & F1 (micro) 
                                   \\ \midrule
            Prior (Most)
            & 26.8
            & 0.27
            & 25.3
            & 0.25 \\
            Prior (Question)
            & 34.2
            & 0.34
            & 32.4
            & 0.32 \\
            PubMedCLIP
            & $53.6_{\text{ ± } 1.0}$ 
            & $0.58_{\text{ ± } 0.01}$ 
            & $53.2_{\text{ ± } 0.1}$ 
            & $0.57_{\text{ ± } 0.01}$ \\
            PubMedCLIP$^{\ast}$
            & $53.6_{\text{ ± } 0.8}$ 
            & $0.57_{\text{ ± } 0.01}$ 
            & $53.4_{\text{ ± } 0.6}$ 
            & $0.57_{\text{ ± } 0.01}$ \\
            MedViLL$^{\ast}$
            & $65.9_{\text{ ± } 0.2}$ 
            & $0.70_{\text{ ± } 0.00}$ 
            & $65.4_{\text{ ± } 0.3}$ 
            & $0.68_{\text{ ± } 0.00}$ \\
            M$^{3}$AE
            & $69.7_{\text{ ± } 0.2}$ 
            & $0.73_{\text{ ± } 0.00}$ 
            & $69.1_{\text{ ± } 0.3}$ 
            & $0.72_{\text{ ± } 0.00}$ \\
            M$^{3}$AE$^{\ast}$
            & $70.7_{\text{ ± } 0.3}$ 
            & $0.74_{\text{ ± } 0.00}$ 
            & $69.7_{\text{ ± } 0.4}$ 
            & $0.73_{\text{ ± } 0.00}$ \\
            \bottomrule
            \end{tabular}%
            }
  \end{table}

==> supp_tabs/vqa_exp_template_content.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{3pt}
    \noindent
    \centering
    \caption{ Comparison of performance (Acc) of models across content types on \textbf{MIMIC-CXR-VQA (\textit{Template})}.}
    \resizebox{0.75\textwidth}{!}{%
        \begin{tabular}{cccccccc}
        \toprule
        \multicolumn{8}{c}{Valid} \\
        \midrule
        Model & Plane & Gender & Size & Abnormality & Anatomy & Attribute & Condition \\
        \midrule
        Prior (Most) 
        & $16.7 $ 
        & $16.7 $ 
        & $50.0 $ 
        & $24.7 $ 
        & $0.0 $ 
        & $0.0 $ 
        & $50.0 $ \\
        Prior (Question) 
        & $50.0 $ 
        & $50.0 $ 
        & $50.0 $ 
        & $29.5 $ 
        & $10.9 $ 
        & $16.9 $ 
        & $50.0 $ \\
        PubMedCLIP 
        & $62.8_{\text{ ± } 0.7}$ 
        & $42.9_{\text{ ± } 1.2}$ 
        & $77.7_{\text{ ± } 0.6}$ 
        & $49.8_{\text{ ± } 0.6}$ 
        & $31.7_{\text{ ± } 1.1}$ 
        & $35.5_{\text{ ± } 0.4}$ 
        & $70.8_{\text{ ± } 0.6}$ \\
        PubMedCLIP$^\ast$ 
        & $61.9_{\text{ ± } 0.7}$ 
        & $43.9_{\text{ ± } 1.1}$ 
        & $77.7_{\text{ ± } 1.1}$ 
        & $50.1_{\text{ ± } 0.4}$ 
        & $32.0_{\text{ ± } 0.5}$ 
        & $35.7_{\text{ ± } 0.2}$ 
        & $70.9_{\text{ ± } 0.3}$ \\
        MedViLL$^\ast$ 
        & $99.0_{\text{ ± } 0.1}$
        & $91.0_{\text{ ± } 0.2}$
        & $76.3_{\text{ ± } 0.5}$
        & $60.4_{\text{ ± } 0.3}$
        & $44.4_{\text{ ± } 0.4}$
        & $56.1_{\text{ ± } 0.1}$
        & $76.7_{\text{ ± } 0.4}$ \\
        M$^{3}$AE 
        & $99.3_{\text{ ± } 0.1}$
        & $94.6_{\text{ ± } 0.3}$
        & $81.7_{\text{ ± } 0.3}$
        & $65.1_{\text{ ± } 0.1}$
        & $48.5_{\text{ ± } 0.1}$
        & $60.8_{\text{ ± } 0.3}$
        & $79.4_{\text{ ± } 0.4}$ \\
        M$^{3}$AE$^\ast$
        & $99.4_{\text{ ± } 0.3}$
        & $93.9_{\text{ ± } 0.5}$
        & $81.9_{\text{ ± } 0.6}$
        & $66.4_{\text{ ± } 0.3}$
        & $50.1_{\text{ ± } 0.5}$
        & $61.9_{\text{ ± } 0.7}$
        & $80.3_{\text{ ± } 0.1}$ \\
        \toprule
        \multicolumn{8}{c}{Test} \\
        \midrule
        Model & Plane & Gender & Size & Abnormality & Anatomy & Attribute & Condition \\
        \midrule
        Prior (Most)
        & $17.1 $ & $16.7 $ & $43.3 $ & $23.9 $ & $0.0 $ & $0.0 $ & $50.4 $ \\
        Prior (Question) 
        & $48.7 $ 
        & $50.0 $
        & $43.3 $ 
        & $28.8 $ 
        & $10.9 $ 
        & $13.1 $ 
        & $50.4 $ \\
        PubMedCLIP
        & $61.3_{\text{ ± } 1.3}$
        & $43.9_{\text{ ± } 0.6}$
        & $75.5_{\text{ ± } 1.1}$
        & $47.7_{\text{ ± } 0.2}$
        & $34.0_{\text{ ± } 1.7}$
        & $35.6_{\text{ ± } 0.5}$
        & $71.4_{\text{ ± } 0.4}$ \\
        PubMedCLIP$^\ast$ 
        & $60.5_{\text{ ± } 1.5}$
        & $44.0_{\text{ ± } 3.2}$
        & $76.2_{\text{ ± } 1.0}$
        & $47.7_{\text{ ± } 0.5}$
        & $34.4_{\text{ ± } 0.8}$
        & $35.8_{\text{ ± } 0.3}$
        & $71.1_{\text{ ± } 1.0}$ \\
        MedViLL$^\ast$ 
        & $99.5_{\text{ ± } 0.3}$
        & $92.0_{\text{ ± } 0.1}$
        & $75.0_{\text{ ± } 0.9}$
        & $60.8_{\text{ ± } 0.2}$
        & $46.7_{\text{ ± } 0.5}$
        & $54.9_{\text{ ± } 0.4}$
        & $76.0_{\text{ ± } 0.3}$ \\
        M$^{3}$AE 
        & $99.1_{\text{ ± } 0.1}$
        & $94.5_{\text{ ± } 0.1}$
        & $81.1_{\text{ ± } 0.5}$
        & $64.2_{\text{ ± } 0.1}$
        & $51.1_{\text{ ± } 0.3}$
        & $60.5_{\text{ ± } 1.1}$
        & $78.6_{\text{ ± } 0.1}$ \\
        M$^{3}$AE$^\ast$ 
        & $99.5_{\text{ ± } 0.3}$
        & $93.3_{\text{ ± } 1.0}$
        & $80.3_{\text{ ± } 1.2}$
        & $65.1_{\text{ ± } 0.2}$
        & $53.2_{\text{ ± } 1.3}$
        & $60.8_{\text{ ± } 0.8}$
        & $78.9_{\text{ ± } 0.3}$ \\
        \bottomrule
    \end{tabular}
    }
\end{table}

